Determinantal sets, singularities and application to optimal control in medical imagery

Control theory has recently been involved in the field of nuclear magnetic resonance imagery. The goal is to control the magnetic field optimally in order to improve the contrast between two biological matters on the pictures. Geometric optimal control leads us here to analyze mero-morphic vector fields depending upon physical parameters , and having their singularities defined by a deter-minantal variety. The involved matrix has polynomial entries with respect to both the state variables and the parameters. Taking into account the physical constraints of the problem, one needs to classify, with respect to the parameters, the number of real singularities lying in some prescribed semi-algebraic set. We develop a dedicated algorithm for real root classification of the singularities of the rank defects of a polynomial matrix, cut with a given semi-algebraic set. The algorithm works under some genericity assumptions which are easy to check. These assumptions are not so restrictive and are satisfied in the aforementioned application. As more general strategies for real root classification do, our algorithm needs to compute the critical loci of some maps, intersections with the boundary of the semi-algebraic domain, etc. In order to compute these objects, the determinantal structure is exploited through a stratifi-cation by the rank of the polynomial matrix. This speeds up the computations by a factor 100. Furthermore, our implementation is able to solve the application in medical imagery, which was out of reach of more general algorithms for real root classification. For instance, computational results show that the contrast problem where one of the matters is water is partitioned into three distinct classes.

==> criticallocus.tex <==

\section{Critical locus of $\{D=0\}\cap\{D'=0\}$}
\label{section:Critical}
Let us define the polynomial $\Xi_2(\gamma_2,\Gamma_2,z_2,y_2^2)$
{\tiny
\[
\begin{array}{l}
\gamma_2\, \left( 2\,\Gamma_2-\gamma_2-2 \right)  \left( \Gamma_2-\gamma_2-
1 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}{z_2^4}+
\\
\gamma_2\,
 \left( \Gamma_2-\gamma_2 \right)  \left( 6\,{\Gamma_2^3}-9\,{\Gamma_2^2}\gamma_2+5\,\Gamma_2\,{\gamma_2^2}-{\gamma_2^3}-12\,{\Gamma_2^2}+
12\,\Gamma_2\,\gamma_2-4\,{\gamma_2^2}+6\,\Gamma_2-3\,\gamma_2 \right) {z_2^3}+
\\
 \left( -2\, \left( {\Gamma_2^3}-{\Gamma_2^2}\gamma_2-
\Gamma_2\,{\gamma_2^2}+{\gamma_2^3}-2\,{\Gamma_2^2}+3\,\Gamma_2\,
\gamma_2-2\,{\gamma_2^2}-\Gamma_2-\gamma_2+2 \right)  \left( \Gamma_2-
\gamma_2 \right) ^{2}{y_2^2}+
\gamma_2\, \left( \Gamma_2-1 \right) 
 \left( 6\,{\Gamma_2^3}-9\,{\Gamma_2^2}\gamma_2+5\,\Gamma_2\,\gamma_2
^{2}-{\gamma_2^3}-6\,{\Gamma_2^2}+6\,\Gamma_2\,\gamma_2-{\gamma_2^2}
 \right)  \right) {z_2^2}+
 \\
  \left( - \left( \Gamma_2-\gamma_2
 \right)  \left( 4\,{\Gamma_2^4}-5\,{\Gamma_2^3}\gamma_2+{\Gamma_2^2}{\gamma_2^2}+\Gamma_2\,{\gamma_2^3}-8\,{\Gamma_2^3}+16\,{\Gamma_2^2}\gamma_2-8\,\Gamma_2\,{\gamma_2^2}-4\,{\Gamma_2^2}-5\,\Gamma_2\,
\gamma_2+4\,{\gamma_2^2}+8\,\Gamma_2-4\,\gamma_2 \right) {y_2^2}+
\Gamma_2\,\gamma_2\, \left( \Gamma_2-1 \right) ^{2} \left( 2\,\Gamma_2-
\gamma_2 \right)  \right) z_2+\Gamma_2\, \left( -\gamma_2+\Gamma_2+1
 \right)  \left( -2\,\gamma_2+\Gamma_2+2 \right)  \left( \Gamma_2-\gamma_2
 \right) ^{2}{y_2^4}- \left( \Gamma_2-1 \right)  \left( {\Gamma_2^2}-2\,\Gamma_2+\gamma_2 \right)  \left( -\gamma_2+\Gamma_2+1 \right) 
 \left( 2\,\Gamma_2-\gamma_2 \right) {y_2^2}
\end{array}
\]
}
\begin{theorem}
\label{thm:projy2z2}
Provided ...
the projection of the critical locus on $(y_2,z_2)$ is a degree $4$ curve defined by $\Xi_2(\gamma_2,\Gamma_2,z_2,y_2^2)=0$.
\end{theorem}


 %\marginpar{\textcolor{red}{A FINIR}}
\vskip2cm

Let us define the polynomial $\Xi_1(\gamma_2,\Gamma_2,z_1,y_1^2)$
{\tiny
\[
\begin{array}{l}
6\,\Gamma_2\, \left( \Gamma_2-\gamma_2 \right) ^{4}y_1^{4}z_1^{4}+\Gamma_2\, \left( -\gamma_2+\Gamma_2+1 \right)  \left( 2\,\Gamma
2-\gamma_2 \right)  \left( \Gamma_2-1 \right) ^{2}z_1\,y_1^{
2}+
\\
4\,\Gamma_2\, \left( \Gamma_2-\gamma_2 \right) ^{4}y_1^{2}z_1^{6}+ \left( 3\,\Gamma_2^{2}-4\,\Gamma_2\,\gamma_2+\Gamma_2+
\gamma_2+1 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}y_1^{6}z_1+ 
\\
\left( \Gamma_2-\gamma_2 \right)  \left( 3\,\Gamma_2^{4}-7\,{
\Gamma_2}^{3}\gamma_2+9\,\Gamma_2^{2}\gamma_2^{2}-4\,\Gamma_2\,{\gamma_2
}^{3}+\Gamma_2^{3}-4\,\Gamma_2^{2}\gamma_2-2\,\Gamma_2\,\gamma_2^{2}+
3\,\gamma_2^{3}-4\,\Gamma_2^{2}+11\,\Gamma_2\,\gamma_2-3\,\gamma_2^{2
}-\Gamma_2-5\,\gamma_2+3 \right) z_1^{3}y_1^{2}+
\\
 \left( 
\Gamma_2-1 \right)  \left( 4\,\Gamma_2^{4}-6\,\Gamma_2^{3}\gamma_2+2\,
\Gamma_2^{2}\gamma_2^{2}-3\,\Gamma_2^{3}+9\,\Gamma_2^{2}\gamma_2-7
\,\Gamma_2\,\gamma_2^{2}+2\,\gamma_2^{3}-6\,\Gamma_2^{2}+8\,\Gamma_2
\,\gamma_2-4\,\gamma_2^{2}-\Gamma_2+2\,\gamma_2 \right) y_1^{2}z_1^{2}- 
\\
\left( \Gamma_2-1 \right) ^{2} \left( \Gamma_2-\gamma_2-1
 \right)  \left( -\gamma_2+\Gamma_2+1 \right) ^{2}z_1^{3}-
\\
 \left( \Gamma_2-1 \right)  \left( -\gamma_2+\Gamma_2+1 \right)  \left( 3
\,\Gamma_2^{3}-5\,\Gamma_2^{2}\gamma_2+\Gamma_2\,\gamma_2^{2}+\gamma_2^{3}
-4\,\Gamma_2^{2}+7\,\Gamma_2\,\gamma_2-3\,\gamma_2^{2}+2\,\Gamma
2-3\,\gamma_2+1 \right) z_1^{4}+
\\
3\, \left( -\gamma_2+\Gamma_2
 \right) ^{2} \left( 2\,\Gamma_2^{3}-4\,\Gamma_2^{2}\gamma_2+2\,
\Gamma_2\,\gamma_2^{2}+2\,\Gamma_2^{2}-\gamma_2^{2}-\Gamma_2+1
 \right) z_1^{2}y_1^{4}
\\
-\Gamma_2^{2} \left( 2\,\Gamma_2-
\gamma_2 \right)  \left( \gamma_2-1 \right)  \left( \Gamma_2-1 \right) y_1^{4}+3\, \left( 3\,\Gamma_2^{2}-4\,\Gamma_2\,\gamma_2+\Gamma_2+
\gamma_2+1 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}y_1^{2}{
z_1}^{5}+
\\
 \left( \Gamma_2-\gamma_2 \right)  \left( 5\,\Gamma_2^{4}-7\,\Gamma_2^{3}\gamma_2+3\,\Gamma_2^{2}\gamma_2^{2}-5\,\Gamma_2^{
3}+8\,\Gamma_2^{2}\gamma_2-5\,\Gamma_2\,\gamma_2^{2}-\Gamma_2^{2}+3\,
\Gamma_2\,\gamma_2+\gamma_2^{2}-\Gamma_2-\gamma_2 \right) y_1^{4}z_1+\Gamma_2\, \left( \Gamma_2-\gamma_2 \right) ^{4}y_1^{8}+
\\
 \left( 3\,\Gamma_2^{2}-4\,\Gamma_2\,\gamma_2+\Gamma_2+\gamma_2+1
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}z_1^{7}+ \left( -
\gamma_2+\Gamma_2 \right) ^{2} \left( 2\,\Gamma_2^{3}-8\,\Gamma_2^{2}
\gamma_2+6\,\Gamma_2\,\gamma_2^{2}+4\,\Gamma_2^{2}-2\,\Gamma_2\,\gamma_2
-3\,\gamma_2^{2}-\Gamma_2+3 \right) z_1^{6}+
\\
4\,\Gamma_2\,
 \left( \Gamma_2-\gamma_2 \right) ^{4}y_1^{6}z_1^{2}-
 \left( \Gamma_2-\gamma_2 \right)  \left( 2\,\Gamma_2^{4}-6\,\Gamma_2
^{2}\gamma_2^{2}+4\,\Gamma_2\,\gamma_2^{3}-6\,\Gamma_2^{3}+12\,{
\Gamma_2}^{2}\gamma_2-3\,\Gamma_2\,\gamma_2^{2}-3\,\gamma_2^{3}+
3\,{
\Gamma_2}^{2}-8\,\Gamma_2\,\gamma_2+4\,\gamma_2^{2}+4\,\gamma_2-3
 \right) z_1^{5}
\\
+\Gamma_2\, \left( -\gamma_2+\Gamma_2+1 \right) 
 \left( \Gamma_2-\gamma_2 \right) ^{2} \left( 2\,\Gamma_2-1 \right) y_1^{6}+
\\
\Gamma_2\, \left( \Gamma_2-\gamma_2 \right) ^{4}z_1^
{8}+3\, \left( \Gamma_2-\gamma_2 \right) ^{2} \left( \Gamma_2-2\,\gamma_2
+2 \right)  \left( 2\,\Gamma_2^{2}-2\,\Gamma_2\,\gamma_2-\Gamma_2+\gamma
2+1 \right) y_1^{2}z_1^{4}+3\, \left( 3\,\Gamma_2^{2}-4
\,\Gamma_2\,\gamma_2+\Gamma_2+\gamma_2+1 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}y_1^{4}z_1^{3}
\end{array}
\]
}
\begin{proposition}
\label{prp:projy1z1}
Provided ...
the projection of the critical locus on $(y_1,z_1)$ is a degree $8$ curve defined by $\Xi_1(\gamma_2,\Gamma_2,z_1,y_1^2)=0$.
\end{proposition}

 %\marginpar{\textcolor{red}{A FINIR}}
\vskip2cm

\subsection{Classification of configurations}
We classify here the different configurations of the zeroes of $\Xi_1$, $\Xi_2$ inside the Bloch ball.

 %\marginpar{\textcolor{red}{A FINIR}}
\vskip2cm


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SingulWater"
%%% End:


==> expressions.tex <==

\section{Rational expressions of $\{D=0\}\cap\{D'=0\}$}
\label{section:Intersection}
In this section we give explicit rational expressions of the (generically) surface $\{D=0\}\cap\{D'=0\}$ and we describe the set of 
non-transversal intersection.



\subsection{Rational expressions of $\{D=0\}\cap\{D'=0\}$}
\label{subsection:ExpressionsIntersec}

Let us introduce the polynomials:
\[
P_1^y(\gamma_2,\Gamma_2,z_2)=
2 \left( \gamma_2-\Gamma_2 \right) z_2-2\,\Gamma_2+\gamma_2
\]
\[
P_1^z(\gamma_2,\Gamma_2,z_2,y_2^2)=
\gamma_2 \left(\gamma_2- \Gamma_2 \right) z_2^2-\Gamma_2\,
\gamma_2\,{z_2}+\Gamma_2 \left( \Gamma_2-\gamma_2 \right) y_2^2
\]
%\[
%Q_1^z(\gamma_2,\Gamma_2,z_2,y_2^2)=\gamma_2\,\left( 1+\gamma_2-\Gamma_2 \right) z_2^2
%+ \gamma_2\,\left(1 -\Gamma_2 \right) z_2+ \Gamma_2\,\left(1+ \Gamma_2-\gamma_2\right) y_2^2
%\]
\[
Q_1^z(\gamma_2,\Gamma_2,z_2,y_2^2)=
\gamma_2\left( \Gamma_2- \gamma_2-1 \right) z_2^2+\gamma_2\, \left( \Gamma_2-1 \right) z_2+
\Gamma_2 \left(\gamma_2 -\Gamma_2-1\right) y_2^2
\]


{\tiny
\[
R_1(\gamma_2,\Gamma_2,z_2,y_2^2)=\gamma_2^2 \left( \Gamma_2-\gamma_2 \right) ^{2}z_2^{4}+2\,\Gamma_2\,\gamma_2^2 \left( \Gamma_2-\gamma_2 \right) z_2^{3}+
\left( 2\, \left(2- \Gamma_2\,\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}y_2^2+\Gamma_2^2\gamma_2^2 \right) {z_2^2}-2\, \left( \Gamma_2^2\gamma_2-4\,\Gamma_2+2\,\gamma_2 \right) 
 \left( \Gamma_2-\gamma_2 \right) y_2^2\,z_2+\Gamma_2^2
 \left( \Gamma_2-\gamma_2 \right) ^{2}y_2^{4}+ \left( 2\,\Gamma_2-\gamma_2 \right) ^{2}y_2^2
\]
}
{\tiny
\[
P_2^z(\gamma_2,\Gamma_2,z_2,y_2^2)=
2\, \left( \Gamma_2-\gamma_2-1 \right)  \left( 2\,\Gamma_2^2-3\,\Gamma_2\,\gamma_2+\gamma_2^2-2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}z_2^{3}
+ \left( 12\,\Gamma_2^{4}-28\,\Gamma_2^{3}\gamma_2+25\,\Gamma_2^2\gamma_2^2-11\,\Gamma_2\,\gamma_2^{3}+2\,\gamma_2^{4}-12\,\Gamma_2^{3}+24\,\Gamma_2^2\gamma_2-17\,\Gamma_2\,
\gamma_2^2+4\,\gamma_2^{3}-12\,\Gamma_2^2+8\,\Gamma_2\,\gamma_2-2\,\gamma_2^2+12\,\Gamma_2-4\,\gamma_2 \right)  \left( \Gamma_2-\gamma_2\right) ^{2}z_2^2
 + \left( -2\, \left( \Gamma_2-\gamma_2+1 \right)  \left( \Gamma_2^2-3\,\Gamma_2\,\gamma_2+2\,\gamma_2^2-2
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}y_2^2+ \left( \Gamma_2-1 \right)  \left( \Gamma_2-\gamma_2 \right)  \left( 2\,\Gamma_2-\gamma_2 \right)  \left( 6\,\Gamma_2^{3}-10\,\Gamma_2^2\gamma_2+6\,\Gamma_2
\,\gamma_2^2-\gamma_2^{3}+2\,\Gamma_2\,\gamma_2-6\,\Gamma_2+\gamma_2\right)  \right) z_2- \left( \Gamma_2^2-2\,\Gamma_2\,\gamma_2+2
\,\gamma_2-2 \right)  \left( \Gamma_2-\gamma_2+1 \right)  \left( 2\,\Gamma_2-\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}y_2^2+
\Gamma_2\, \left( \Gamma_2-1 \right) ^{2} \left( \Gamma_2-\gamma_2+1 \right)  \left( 2\,\Gamma_2-\gamma_2 \right) ^{2}
\]
}
{\tiny
\[
P_2^y=
(\gamma_2,\Gamma_2,z_2,y_2^2)=2\, \left( \Gamma_2-\gamma_2-1 \right)  \left( 2\,\Gamma_2^2-3\,\Gamma_2\,\gamma_2+\gamma_2^2-2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}z_2^{3}
 + \left( 12\,\Gamma_2^{4}-28\,\Gamma_2^{3}\gamma_2+25\,\Gamma_2^2\gamma_2^2-11\,\Gamma_2\,\gamma_2^{3}+2\,
\gamma_2^{4}-12\,\Gamma_2^{3}+24\,\Gamma_2^2\gamma_2-17\,\Gamma_2\,\gamma_2^2+4\,\gamma_2^{3}-12\,\Gamma_2^2+8\,\Gamma_2\,\gamma_2-2\,\gamma_2^2+12\,\Gamma_2-4\,\gamma_2 \right)  \left( \Gamma_2-\gamma_2\right) ^{2}z_2^2
 + \left( -2\, \left( \Gamma_2-\gamma_2+1
 \right)  \left( \Gamma_2^2-3\,\Gamma_2\,\gamma_2+2\,\gamma_2^2-2
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}Y_2+ \left( \Gamma_2-1 \right)  \left( \Gamma_2-\gamma_2 \right)  \left( 2\,\Gamma_2-\gamma_2 \right)  \left( 6\,\Gamma_2^{3}-10\,\Gamma_2^2\gamma_2+6\,\Gamma_2
\,\gamma_2^2-\gamma_2^{3}+2\,\Gamma_2\,\gamma_2-6\,\Gamma_2+\gamma_2
 \right)  \right) z_2- 
 \left( \Gamma_2^2-2\,\Gamma_2\,\gamma_2+2\,\gamma_2-2 \right)  \left( \Gamma_2-\gamma_2+1 \right)  \left( 2\,\Gamma_2-\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}y_2^2+
\Gamma_2\, \left( \Gamma_2-1 \right) ^{2} \left( \Gamma_2-\gamma_2+1 \right)  \left( 2\,\Gamma_2-\gamma_2 \right) ^{2}
\]
}
{\tiny
\[
R_2(\gamma_2,\Gamma_2,z_2,y_2^2)=4\, \left( \Gamma_2-\gamma_2-1 \right) ^{2} \left( \Gamma_2-\gamma_2
 \right) ^{4}z_2^{4}+4\, \left( \Gamma_2-\gamma_2-1 \right) 
 \left( 4\,\Gamma_2^2-3\,\Gamma_2\,\gamma_2+\gamma_2^2-4\,\Gamma_2+
\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{3}z_2^{3}+
 \left( -4\, \left( \Gamma_2^2-2\,\Gamma_2\,\gamma_2+\gamma_2^2-2
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{4}y_2^2+ \left( 24\,{
\Gamma_2^4}-36\,\Gamma_2^{3}\gamma_2+21\,\Gamma_2^2\gamma_2^2-6
\,\Gamma_2\,\gamma_2^{3}+\gamma_2^{4}-48\,\Gamma_2^{3}+48\,{\Gamma_2^2}\gamma_2-18\,\Gamma_2\,\gamma_2^2+2\,\gamma_2^{3}+24\,\Gamma_2^2-12\,\Gamma_2\,\gamma_2+\gamma_2^2 \right)  \left( \Gamma_2-\gamma_2
 \right) ^{2} \right) z_2^2+ \left( -4\, \left( 2\,\Gamma_2^
{3}-4\,\Gamma_2^2\gamma_2+3\,\Gamma_2\,\gamma_2^2-\gamma_2^{3}+2
\,\Gamma_2\,\gamma_2-4\,\Gamma_2+\gamma_2 \right)  \left( \Gamma_2-\gamma_2
 \right) ^{3}y_2^2+2\,\Gamma_2\, \left( \Gamma_2-1 \right)  \left( 
\Gamma_2-\gamma_2 \right)  \left( 2\,\Gamma_2-\gamma_2 \right)  \left( 4\,
\Gamma_2^2-3\,\Gamma_2\,\gamma_2+\gamma_2^2-4\,\Gamma_2+\gamma_2
 \right)  \right) z_2+4\, \left( \Gamma_2-\gamma_2+1 \right) ^{2}
 \left( \Gamma_2-\gamma_2 \right) ^{4}y_2^{4}-\Gamma_2\, \left( 2
\,\Gamma_2^2-3\,\Gamma_2\,\gamma_2+4\,\gamma_2-4 \right)  \left( 2\,
\Gamma_2-\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}y_2^2+{
\Gamma_2^2} \left( \Gamma_2-1 \right) ^{2} \left( 2\,\Gamma_2-\gamma_2\right) ^{2}
\]
}

Observe that $R_1,R_2,P_2^z$ are of degree $4$ in $z_2$ and $y_2$, $P_2^y$ is of degree $3$ in $z_2$, $Q_1^z,P_1^z,$ are quadratic. 


\begin{theorem}
\label{thm:intersec}
Provided 
%$\gamma_2 \ldots \Gamma_2\ldots $, and 
$R_1(\gamma_2,\Gamma_2,z_2,y_2^2)R_2(\gamma_2,\Gamma_2,z_2,y_2^2) \neq 0$,
$\{D=0\}\cap\{D'=0\}$ is the union of two rational surfaces
\[
\xi_1 : 
\left\{ 
\begin{array}{rl}
z_1=&\frac{P_1^z(\gamma_2,\Gamma_2,z_2,y_2^2)\,Q_1^z(\gamma_2,\Gamma_2,z_2,y_2^2) }{R_1(\gamma_2,\Gamma_2,z_2,y_2^2)}
\\
y_1=&\frac{P_1^y(\gamma_2,\Gamma_2,z_2)\,Q_1^z(\gamma_2,\Gamma_2,z_2,y_2^2)}{R_1(\gamma_2,\Gamma_2,z_2,y_2^2)}\,y_2
\end{array}
\right.
\text{ and }
\xi_2 : 
\left\{
\begin{array}{rl}
z_1=&\frac{P_2^z(\gamma_2,\Gamma_2,z_2,y_2^2)}{R_2(\gamma_2,\Gamma_2,z_2,y_2^2)}
\\
y_1=&\frac{P_2^y(\gamma_2,\Gamma_2,z_2,y_2^2)}{R_2(\gamma_2,\Gamma_2,z_2,y_2^2)}\,y_2
\end{array}
\right.
\]
where $P_1^z,P_1^y,Q_1^z,P_2^z,P_2^y$ correspond to the polynomials defined above.
%The formulas are explicit in terms of $\Gamma_2,\gamma_2,z_2,y_2$.

\end{theorem}
We do not care with points which are at infinity, since we only consider points inside the Bloch ball.
it should be observed that the two surfaces are given by a rational parametrization, which is not always the case (for instance in the blood case, $\gamma_2=\gamma_1$, only one surface is given by an explicit rational expression).





\subsection{Proof of Theorem~\ref{thm:intersec}}
\label{subsection:intersec}

\begin{proof}
The resultant of $D$ and $D'$  with respect to $y_1$ is a product of two polynomials, and each of them is of degree $1$ in $z_1$.
Provided $R_1(\gamma_2,\Gamma_2,z_2,y_2^2) \, R_2(\gamma_2,\Gamma_2,z_2,y_2^2 ) \neq 0$, we can solve each polynomial with respect to $z_1$, 
and get the corresponding expressions given in the statement.
Substituting each of these expressions in $\{ D=0,D'=0\}$ leads to the expressions given above for $y_1$.

We now consider the case $R_1(\gamma_2,\Gamma_2,z_2,y_2^2) \, R_2(\gamma_2,\Gamma_2,z_2,y_2^2 ) =0$,
%\marginpar{\textcolor{red}{A FINIR}}



\vskip4cm
\iffalse%%%%%%%%%%%%%%%%%%%%%%%%%%%
The first surface is given by:
{\tiny
\[
 t={\frac { \left(  \left( 2\,\Gamma_2-2\,\gamma_2 \right) {z_2}+2\,\Gamma_2-\gamma_2 \right)  \left( -\gamma_2\, \left( \Gamma_2-\gamma_2-1 \right) z_2^2-\gamma_2\, \left( \Gamma_2-1
 \right) z_2+\Gamma_2\, \left( \Gamma_2-\gamma_2+1 \right) {
Y_2} \right) }{\gamma_2^2 \left( \Gamma_2-\gamma_2 \right) ^{2}z_2^{4}+2\,\Gamma_2\,\gamma_2^2 \left( \Gamma_2-\gamma_2
 \right) z_2^{3}+ \left( -2\, \left( \Gamma_2\,\gamma_2-2
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}Y_2+\Gamma_2^2
\gamma_2^2 \right) z_2^2-2\, \left( \Gamma_2^2\gamma_2-4\,\Gamma_2+2\,\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) Y_2\,z_2+\Gamma_2^2 \left( \Gamma_2-\gamma_2 \right) ^{2}
Y_2^2+ \left( 2\,\Gamma_2-\gamma_2 \right) ^{2}Y_2}}
\]
\[
{z_1}=-{\frac { \left( -\gamma_2\, \left( \Gamma_2-\gamma_2 \right) 
z_2^2-\gamma_2\,z_2\,\Gamma_2+\Gamma_2\, \left( \Gamma_2
-\gamma_2 \right) Y_2 \right)  \left( -\gamma_2\, \left( \Gamma_2
-\gamma_2-1 \right) z_2^2-\gamma_2\, \left( \Gamma_2-1
 \right) z_2+\Gamma_2\, \left( \Gamma_2-\gamma_2+1 \right) {Y_2} \right) }{\gamma_2^2 \left( \Gamma_2-\gamma_2 \right) ^{2}z_2^{4}+2\,\Gamma_2\,\gamma_2^2 \left( \Gamma_2-\gamma_2
 \right) z_2^{3}+ \left( -2\, \left( \Gamma_2\,\gamma_2-2
 \right)  \left( \Gamma_2-\gamma_2 \right) ^{2}Y_2+\Gamma_2^2
\gamma_2^2 \right) z_2^2-2\, \left( \Gamma_2^2\gamma_2-4\,\Gamma_2+2\,\gamma_2 \right)  \left( \Gamma_2-\gamma_2 \right) {Y_2}\,z_2+\Gamma_2^2 \left( \Gamma_2-\gamma_2 \right) ^{2}
Y_2^2+ \left( 2\,\Gamma_2-\gamma_2 \right) ^{2}Y_2}}
\]
\fi%%%%%%%%%%%%%%%%%%
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "SingulWater"
%%% End:

